Moduli spaces of slope-semistable pure sheaves

We construct a moduli space of slope-semistable pure sheaves, building upon previous work of Le Potier and Jun Li on torsion-free sheaves over smooth surfaces. In particular, our construction provides a compactification of the Simpson moduli space of slope-stable reflexive sheaves. We also prove an effective restriction theorem for slope-(semi)stable pure sheaves following an approach due to Langer.

==> tex/Aknowledgments.tex <==
\subsection*{Acknowledgements}

The author wishes to express his gratitude to his supervisor, Prof.~Matei Toma, for his patient guidance and fruitful discussions during the preparation of this paper, which will be part of the author's PhD thesis. The author wishes to thank Adrian Langer for his helpful comments on a preliminary version of this paper.
